On the cosmological mass function theory

This paper provides, from one side, a review of the theory of the cosmological mass function from a theoretical point of view, starting from the seminal paper of Press & Shechter (1974) to the last developments (Del Popolo & Gambera (1998, 1999), Sheth & Tormen 1999 (ST), Sheth, Mo & Tormen 2001 (ST1), Jenkins et al. 2001 (J01), Shet & Tormen 2002 (ST2), Del Popolo 2002a, Yagi et al. 2004 (YNY)), and from another side some improvements on the multiplicity function models in literature. ...

==> epsfig.tex <==
%%
%% This is file `epsfig.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% epsfig.dtx  (with options: `package')
%% 
%% epsfig.dtx Copyright (C) 1994-1996 Sebastian Rahtz
%%
%% This file is part of the Standard LaTeX `Graphics Bundle'.
%%
%% It should be distributed *unchanged* and together with all other
%% files in the graphics bundle. The file 00readme.txt contains a list
%% of all of these files.
%%
%% A modified version of this file may be distributed, but it should
%% be distributed with a *different* name. Changed files must be
%% distributed *together with a complete and unchanged* distribution
%% of these files.
%%
\NeedsTeXFormat{LaTeX2e}[1994/06/01]
\ProvidesPackage{epsfig}
                  [1996/10/04 v1.7 (e)psfig emulation (SPQR)]
\DeclareOption*{\PassOptionsToPackage{\CurrentOption}{graphicx}}
\ProcessOptions
\RequirePackage{graphicx}
\def\psfig#1{%
 \let\Gin@ewidth\Gin@exclamation\let\Gin@eheight\Gin@ewidth
 \def\Gin@req@sizes{%
   \def\Gin@scalex{1}\let\Gin@scaley\Gin@exclamation
   \Gin@req@height\Gin@nat@height
   \Gin@req@width\Gin@nat@width}%
   \begingroup
    \let\Gfigname\relax
    \@tempswafalse
    \toks@{\Ginclude@graphics{\Gfigname}}%
    \setkeys{Gin}{#1}%
    \Gin@esetsize
    \ifx\Gfigname\relax\ErrorNoFile\else
      \the\toks@
    \fi
  \endgroup}
\define@key{Gin}{figure}{\def\Gfigname{#1}}
\define@key{Gin}{file}{\def\Gfigname{#1}}
\define@key{Gin}{prolog}{\typeout{epsfig: header files are not needed}}
\define@key{Gin}{silent}[]{}
\def\psdraft{\Gin@drafttrue}
\def\psfull{\Gin@draftfalse}
\def\pssilent{\typeout{epsfig option `silent' ignored}}
\def\psnoisy{\typeout{epsfig option `noisy' ignored}}
\let\epsfig\psfig
\def\psfigdriver#1{\makeatletter\input{#1.def}\makeatother}
\newdimen\epsfxsize
\newdimen\epsfysize
\epsfysize\z@
\epsfxsize\z@
\def\epsfsize#1#2{\epsfxsize}
\def\epsfbox{%
 \@ifnextchar[%
  {\Gin@bboxtrue\epsf@bb@box}%
  {\Gin@bboxfalse\epsf@box}%
}
\def\epsf@bb@box[#1#2]{%
  \expandafter\Gread@parse@bb#1#2 \\
  \epsf@box}
\def\epsf@box#1{%
 \bgroup
   \def\Gin@req@sizes{%
        \epsfxsize\epsfsize{\Gin@nat@width}{\Gin@nat@height}%
        \ifdim\epsfxsize=\z@
            \ifdim\epsfysize=\z@
                \Gin@req@height\Gin@nat@height
                \Gin@req@width\Gin@nat@width
            \else
                \let\Gin@scalex\Gin@exclamation
                \Gin@req@height\epsfysize
                \Gscale@div\Gin@scaley\Gin@req@height\Gin@nat@height
                \Gin@req@width\Gin@scaley\Gin@nat@width
            \fi
        \else
            \Gin@req@width\epsfxsize
            \Gscale@div\Gin@scalex\Gin@req@width\Gin@nat@width
            \ifdim\epsfysize=\z@
                \let\Gin@scaley\Gin@exclamation
                \Gin@req@height\Gin@scalex\Gin@nat@height
            \else
                \Gin@req@height\epsfysize
                \Gscale@div\Gin@scaley\Gin@req@height\Gin@nat@height
            \fi
        \fi
      }%
 \Ginclude@graphics{#1}%
 \egroup
 \epsfysize\z@
 \epsfxsize\z@
}
\let\epsffile\epsfbox
\def\epsfclipon{\Gin@cliptrue}
\def\epsfclipoff{\Gin@clipfalse}
\def\epsfverbosetrue{\typeout{epsf verbose option ignored}}
\def\epsfverbosefalse{\typeout{epsf verbose option ignored}}

\endinput
%%
%% End of file `epsfig.sty'.

